Exo-SIR: An Epidemiological Model to Analyze the Impact of Exogenous Infection of COVID-19 in India

Epidemiological models are the mathematical models that capture the dynamics of epidemics. The spread of the virus has two routes - exogenous and endogenous. The exogenous spread is from outside the population under study, and endogenous spread is within the population under study. Although some of the models consider the exogenous source of infection, they have not studied the interplay between exogenous and endogenous spreads. In this paper, we introduce a novel model - the Exo-SIR model that captures both the exogenous and endogenous spread of the virus. We analyze to find out the relationship between endogenous and exogenous infections during the Covid19 pandemic. First, we simulate the Exo-SIR model without assuming any contact network for the population. Second, simulate it by assuming that the contact network is a scale free network. Third, we implemented the Exo-SIR model on a real dataset regarding Covid19. We found that endogenous infection is influenced by even a minimal rate of exogenous infection. Also, we found that in the presence of exogenous infection, the endogenous infection peak becomes higher, and the peak occurs earlier. This means that if we consider our response to a pandemic like Covid19, we should be prepared for an earlier and higher number of cases than the SIR model suggests if there are the exogenous source(s) of infection.

==> dump.tex <==
@article{guille2013information,
  title={Information diffusion in online social networks: A survey},
  author={Guille, Adrien and Hacid, Hakim and Favre, Cecile and Zighed, Djamel A},
  journal={ACM Sigmod Record},
  volume={42},
  number={2},
  pages={17--28},
  year={2013},
  publisher={ACM}
}

@article{goldenberg2001talk,
	title={Talk of the network: A complex systems look at the underlying process of word-of-mouth},
	author={Goldenberg, Jacob and Libai, Barak and Muller, Eitan},
	journal={Marketing letters},
	volume={12},
	number={3},
	pages={211--223},
	year={2001},
	publisher={Springer}
}

@article{granovetter1978threshold,
	title={Threshold models of collective behavior},
	author={Granovetter, Mark},
	journal={American journal of sociology},
	volume={83},
	number={6},
	pages={1420--1443},
	year={1978},
	publisher={University of Chicago Press}
}

@article{hethcote2000mathematics,
	title={The mathematics of infectious diseases},
	author={Hethcote, Herbert W},
	journal={SIAM review},
	volume={42},
	number={4},
	pages={599--653},
	year={2000},
	publisher={SIAM}
}

@article{newman2003structure,
	title={The structure and function of complex networks},
	author={Newman, Mark EJ},
	journal={SIAM review},
	volume={45},
	number={2},
	pages={167--256},
	year={2003},
	publisher={SIAM}
}

@article{kumar2019infections,
	title={Infections among Contacts of Patients with Nipah Virus, India},
	author={Kumar, CP Girish and Sugunan, Attayur P and Yadav, Pragya and Kurup, Karishma Krishna and Aarathee, Renjith and Manickam, Ponnaiah and Bhatnagar, Tarun and Radhakrishnan, Chandni and Thomas, Beena and Kumar, Akhilesh and others},
	journal={Emerging infectious diseases},
	volume={25},
	number={5},
	pages={1007},
	year={2019},
	publisher={Centers for Disease Control and Prevention}
}

@article{rahman2012nipah,
	title={Nipah virus outbreaks in Bangladesh: a deadly infectious disease},
	author={Rahman, Mahmudur and Chakraborty, Apurba and others},
	journal={WHO South-East Asia journal of public health},
	volume={1},
	number={2},
	pages={208},
	year={2012},
	publisher={Medknow Publications}
}

@article{chadha2006nipah,
	title={Nipah virus-associated encephalitis outbreak, Siliguri, India},
	author={Chadha, Mandeep S and Comer, James A and Lowe, Luis and Rota, Paul A and Rollin, Pierre E and Bellini, William J and Ksiazek, Thomas G and Mishra, Akhilesh C},
	journal={Emerging infectious diseases},
	volume={12},
	number={2},
	pages={235},
	year={2006},
	publisher={Centers for Disease Control and Prevention}
}

@article{parashar2000case,
	title={Case-control study of risk factors for human infection with a new zoonotic paramyxovirus, Nipah virus, during a 1998--1999 outbreak of severe encephalitis in Malaysia},
	author={Parashar, Umesh D and Sunn, Lye Munn and Ong, Flora and Mounts, Anthony W and Arif, Mohamad Taha and Ksiazek, Thomas G and Kamaluddin, Muhammad A and Mustafa, Amal N and Kaur, Hanjeet and Ding, Lay Ming and others},
	journal={The Journal of infectious diseases},
	volume={181},
	number={5},
	pages={1755--1759},
	year={2000},
	publisher={The University of Chicago Press}
}

@Article{Luby2009,
	author={Luby, Stephen P.
	and Hossain, M. Jahangir
	and Gurley, Emily S.
	and Ahmed, Be Nazir
	and Banu, Shakila
	and Khan, Salah Uddin
	and Homaira, Nusrat
	and Rota, Paul A.
	and Rollin, Pierre E.
	and Comer, James A.
	and Kenah, Eben
	and Ksiazek, Thomas G.
	and Rahman, Mahmudur},
	title={Recurrent zoonotic transmission of Nipah virus into humans, Bangladesh, 2001-2007},
	journal={Emerging infectious diseases},
	year={2009},
	month={Aug},
	publisher={Centers for Disease Control and Prevention},
	volume={15},
	number={8},
	pages={1229-1235},
	note={19751584[pmid]},
	note={PMC2815955[pmcid]},
	issn={1080-6059},
	doi={10.3201/eid1508.081237},
	url={https://www.ncbi.nlm.nih.gov/pubmed/19751584}
}

@inproceedings{myers2012information,
	title={Information diffusion and external influence in networks},
	author={Myers, Seth A and Zhu, Chenguang and Leskovec, Jure},
	booktitle={Proceedings of the 18th ACM SIGKDD international conference on Knowledge discovery and data mining},
	pages={33--41},
	year={2012},
	organization={ACM}
}

@inproceedings{li2015measuring,
	title={Measuring the external influence in information diffusion},
	author={Li, Jiang and Xiong, Jiagui and Wang, Xiaojie},
	booktitle={2015 16th IEEE International Conference on Mobile Data Management},
	volume={2},
	pages={92--97},
	year={2015},
	organization={IEEE}
}

@article{yang2019modeling,
	title={Modeling Information Diffusion with the External Environment in Social Networks},
	author={Yang, Dingda and Liao, Xiangwen and Wei, Jingjing and Chen, Guolong and Cheng, Xueqi},
	journal={Journal of Internet Technology},
	volume={20},
	number={2},
	pages={369--377},
	year={2019}
}

@article{fujita2018identifying,
	title={Identifying exogenous and endogenous activity in social media},
	author={Fujita, Kazuki and Medvedev, Alexey and Koyama, Shinsuke and Lambiotte, Renaud and Shinomoto, Shigeru},
	journal={Physical Review E},
	volume={98},
	number={5},
	pages={052304},
	year={2018},
	publisher={APS}
}

@inproceedings{de2018demarcating,
	title={Demarcating endogenous and exogenous opinion diffusion process on social networks},
	author={De, Abir and Bhattacharya, Sourangshu and Ganguly, Niloy},
	booktitle={Proceedings of the 2018 World Wide Web Conference},
	pages={549--558},
	year={2018},
	organization={International World Wide Web Conferences Steering Committee}
}

@inproceedings{agrawal2012learning,
	title={Learning the nature of information in social networks},
	author={Agrawal, Rakesh and Potamias, Michalis and Terzi, Evimaria},
	booktitle={Sixth International AAAI Conference on Weblogs and Social Media},
	year={2012}
}

@article{oka2014self,
	title={Self-organization on social media: Endo-exo bursts and baseline fluctuations},
	author={Oka, Mizuki and Hashimoto, Yasuhiro and Ikegami, Takashi},
	journal={PloS one},
	volume={9},
	number={10},
	pages={e109293},
	year={2014},
	publisher={Public Library of Science}
}

@article{crane2008robust,
	title={Robust dynamic classes revealed by measuring the response function of a social system},
	author={Crane, Riley and Sornette, Didier},
	journal={Proceedings of the National Academy of Sciences},
	volume={105},
	number={41},
	pages={15649--15653},
	year={2008},
	publisher={National Acad Sciences}
}


@book{bailey1975mathematical,
	title={The mathematical theory of infectious diseases and its applications},
	author={Bailey, Norman TJ and others},
	year={1975},
	publisher={Charles Griffin \& Company Ltd, 5a Crendon Street, High Wycombe, Bucks HP13 6LE.}
}

@inproceedings{de2018demarcating,
	title={Demarcating endogenous and exogenous opinion diffusion process on social networks},
	author={De, Abir and Bhattacharya, Sourangshu and Ganguly, Niloy},
	booktitle={Proceedings of the 2018 World Wide Web Conference},
	pages={549--558},
	year={2018},
	organization={International World Wide Web Conferences Steering Committee}
}

@inproceedings{agrawal2012learning,
	title={Learning the nature of information in social networks},
	author={Agrawal, Rakesh and Potamias, Michalis and Terzi, Evimaria},
	booktitle={Sixth International AAAI Conference on Weblogs and Social Media},
	year={2012}
}

@article{fujita2018identifying,
	title={Identifying exogenous and endogenous activity in social media},
	author={Fujita, Kazuki and Medvedev, Alexey and Koyama, Shinsuke and Lambiotte, Renaud and Shinomoto, Shigeru},
	journal={Physical Review E},
	volume={98},
	number={5},
	pages={052304},
	year={2018},
	publisher={APS}
}

@article{tomasello2014role,
	title={The role of endogenous and exogenous mechanisms in the formation of R\&D networks},
	author={Tomasello, Mario V and Perra, Nicola and Tessone, Claudio J and Karsai, M{\'a}rton and Schweitzer, Frank},
	journal={Scientific reports},
	volume={4},
	pages={5679},
	year={2014},
	publisher={Nature Publishing Group}
}

@article{rizoiu2016can,
	title={Can this video be promoted? Endogenous and exogenous popularity processes in social media},
	author={Rizoiu, Marian-Andrei and Xie, Lexing and Sanner, Scott and Cebrian, Manuel and Yu, Honglin and Van Hentenryck, Pascal},
	journal={arXiv preprint arXiv:1602.06033},
	year={2016}
}

@article{oka2014self,
	title={Self-organization on social media: Endo-exo bursts and baseline fluctuations},
	author={Oka, Mizuki and Hashimoto, Yasuhiro and Ikegami, Takashi},
	journal={PloS one},
	volume={9},
	number={10},
	pages={e109293},
	year={2014},
	publisher={Public Library of Science}
}

@article{crane2008robust,
	title={Robust dynamic classes revealed by measuring the response function of a social system},
	author={Crane, Riley and Sornette, Didier},
	journal={Proceedings of the National Academy of Sciences},
	volume={105},
	number={41},
	pages={15649--15653},
	year={2008},
	publisher={National Acad Sciences}
}

@article{barabasi1999emergence,
	title={Emergence of scaling in random networks},
	author={Barab{\'a}si, Albert-L{\'a}szl{\'o} and Albert, R{\'e}ka},
	journal={science},
	volume={286},
	number={5439},
	pages={509--512},
	year={1999},
	publisher={American Association for the Advancement of Science}
}

@article{li2017survey,
	title={A survey on information diffusion in online social networks: Models and methods},
	author={Li, Mei and Wang, Xiang and Gao, Kai and Zhang, Shanshan},
	journal={Information},
	volume={8},
	number={4},
	pages={118},
	year={2017},
	publisher={Multidisciplinary Digital Publishing Institute}
}

@misc{wilensky1999netlogo,
	title={NetLogo http://ccl.northwestern.edu/netlogo/ (visited 04/01/2020)},
	author={Wilensky, U},
	year={1999}
}

@inproceedings{marcus2011twitinfo,
	title={Twitinfo: aggregating and visualizing microblogs for event exploration},
	author={Marcus, Adam and Bernstein, Michael S and Badar, Osama and Karger, David R and Madden, Samuel and Miller, Robert C},
	booktitle={Proceedings of the SIGCHI conference on Human factors in computing systems},
	pages={227--236},
	year={2011},
	organization={ACM}
}


 @unpublished{WHOReport2020,
	author = {WHO},
	title = {Coronavirus disease 2019 (COVID-19)Situation Report -- 68, www.who.int/docs/default-source/coronaviruse/situation-reports/20200320-sitrep-60-covid-19.pdf},
	date = {29th March, 2020},
	url = {https://www.who.int/docs/default-source/coronaviruse/situation-reports/20200320-sitrep-60-covid-19.pdf}
}

@unpublished{Wiki2020,
	author = {Wikipedia},
	title = {Timeline of the 2020 coronavirus pandemic in India, en.wikipedia.org/wiki/Timeline\_of\_the\_2020\_coronavirus\_pandemic\_in\_India},
	date = {29th March, 2020},
	url = \url{https://en.wikipedia.org/wiki/Timeline\_of\_the\_2020\_coronavirus\_pandemic\_in\_India}
}

@unpublished{CNBC2020,
	author = {Saheli Roy Choudhury, CNBC},
	title = {India temporarily suspends almost all visas and closes land border with Myanmar, https://www.cnbc.com/2020/03/12/coronavirus-india-suspends-most-visas-closes-land-border-with-myanmar.html},
	date = {29th March, 2020},
	url = \url{India temporarily suspends almost all visas and closes land border with Myanmar, \url{https://www.cnbc.com/2020/03/12/coronavirus-india-suspends-most-visas-closes-land-border-with-myanmar.html}}
}

@article{fujita2018identifying,
	title={Identifying exogenous and endogenous activity in social media},
	author={Fujita, Kazuki and Medvedev, Alexey and Koyama, Shinsuke and Lambiotte, Renaud and Shinomoto, Shigeru},
	journal={Physical Review E},
	volume={98},
	number={5},
	pages={052304},
	year={2018},
	publisher={APS}
}

@unpublished{NirmalSynchrony2020,
	author = {Nirmal Kumar S, Sakthi Balan M, Pushkal Agarwal and Lokesh Todwal},
	title = {Social Synchrony in Online Social Networks and its Application in Event Detection from Twitter Data},
	date = {29-03-2020},
}

@article{kermack1927contribution,
	title={A contribution to the mathematical theory of epidemics},
	author={Kermack, William Ogilvy and McKendrick, Anderson G},
	journal={Proceedings of the royal society of london. Series A, Containing papers of a mathematical and physical character},
	volume={115},
	number={772},
	pages={700--721},
	year={1927},
	publisher={The Royal Society London}
}

@incollection{hethcote1989three,
	title={Three basic epidemiological models},
	author={Hethcote, Herbert W},
	booktitle={Applied mathematical ecology},
	pages={119--144},
	year={1989},
	publisher={Springer}
}

@inproceedings{myers2012information,
	title={Information diffusion and external influence in networks},
	author={Myers, Seth A and Zhu, Chenguang and Leskovec, Jure},
	booktitle={Proceedings of the 18th ACM SIGKDD international conference on Knowledge discovery and data mining},
	pages={33--41},
	year={2012},
	organization={ACM}
}
@article{yang2019modeling,
	title={Modeling Information Diffusion with the External Environment in Social Networks},
	author={Yang, Dingda and Liao, Xiangwen and Wei, Jingjing and Chen, Guolong and Cheng, Xueqi},
	journal={Journal of Internet Technology},
	volume={20},
	number={2},
	pages={369--377},
	year={2019}
}

@article{fujita2018identifying,
	title={Identifying exogenous and endogenous activity in social media},
	author={Fujita, Kazuki and Medvedev, Alexey and Koyama, Shinsuke and Lambiotte, Renaud and Shinomoto, Shigeru},
	journal={Physical Review E},
	volume={98},
	number={5},
	pages={052304},
	year={2018},
	publisher={APS}
}
@inproceedings{li2015measuring,
	title={Measuring the external influence in information diffusion},
	author={Li, Jiang and Xiong, Jiagui and Wang, Xiaojie},
	booktitle={2015 16th IEEE International Conference on Mobile Data Management},
	volume={2},
	pages={92--97},
	year={2015},
	organization={IEEE}
}

@article{li2017survey,
	title={A survey on information diffusion in online social networks: Models and methods},
	author={Li, Mei and Wang, Xiang and Gao, Kai and Zhang, Shanshan},
	journal={Information},
	volume={8},
	number={4},
	pages={118},
	year={2017},
	publisher={Multidisciplinary Digital Publishing Institute}
}

@unpublished{MinistryOfHFW2020,
	author = {Ministry of Health and Family Welfare},
	title = {There is enough of everything, everyday for everyone, \url{https://www.mohfw.gov.in/pdf/socialdistancingEnglish.pdf}},
	date = {8th May, 2020},
	url = \url{https://www.mohfw.gov.in/pdf/socialdistancingEnglish.pdf}
} 

@article{szabo2020propagation,
  title={Propagation and mitigation of epidemics in a scale-free network},
  author={Szab{\'o}, Gyula M},
  journal={arXiv preprint arXiv:2004.00067},
  year={2020}
}

@article{fenichel2011adaptive,
  title={Adaptive human behavior in epidemiological models},
  author={Fenichel, Eli P and Castillo-Chavez, Carlos and Ceddia, M Graziano and Chowell, Gerardo and Parra, Paula A Gonzalez and Hickling, Graham J and Holloway, Garth and Horan, Richard and Morin, Benjamin and Perrings, Charles and others},
  journal={Proceedings of the National Academy of Sciences},
  volume={108},
  number={15},
  pages={6306--6311},
  year={2011},
  publisher={National Acad Sciences}
}

@book{barabasi2016network,
  title={Network science},
  author={Barab{\'a}si, Albert-L{\'a}szl{\'o} and others},
  year={2016},
  publisher={Cambridge university press}
}
